Di5Guise: 5G Privacy with vSIM

SIM cards have been the key building block of user authenticationand security in cellular networks. While they are meant to serve as privacy protecting elements in cellular communications, they can be the root cause of privacy loss. Current eSIMs come with a fixed device profile--comprising a secret key, a certificate, and a unique eUICC identifier--that permanently binds every subscriber profile provisioned on the device to that device profile. This binding enables an attacker with the vantage point of a cellular operator to correlate subscriber identities back to a single device, piecing together a complete pattern of life--online activities, movement patterns, and real-world identity--even when users rotate subscriber identities or employ traffic obfuscation techniques. To mitigate this concern, we introduce Di5Guise, a privacy-enhancing architecture that breaks this correlation at its root by decoupling the device identity from the subscriber identity. Central to Di5Guise is vSIM, a virtualized SIM card that enables dynamic device profile provisioning, allowing each subscriber profile to be associated with a distinct, unlinkable device profile. Di5Guise establishes trust with the operator by ensuring that vSIM is running on secure hardware in a trustworthy state. We prototype Di5Guise on a Field Programmable Gate Array (FPGA) board and integrate it with srsRAN to demonstrate full compatibility with existing 5G infrastructure. Using a complex user correlation model, we show that Di5Guise reduces user re-identification accuracy from 93% to 49% when combined with obfuscation.

==> sec/abstract.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract






==> sec/arch.tex <==
\section{\PaperName{} Architecture}
% Architecture Section structure:
% vSIM
%   - Runs in TEE
%   - Interfaces
%   - Just the application 
% Establishing Chain of Trust
%   - HW -> Boot Loader -> Security Monitor -> Driver (can take attestation measurement) -> Application (vSIM)
%   - Platform vSIM runs on (which is part of secure boot process)
%   - Secure Boot (to get to vSIM)
%       (Trust HW (group keys)
% Device Profile Provisioning
%   - Provider SW component + UE Software component
%   - Remote Attestation
%   - Secure Channel Establishment
%   - Security Guarantees (inside threat model?)
%   - Device Profile Switching
% Run-time Operation
%  - 5G Authentication (assume device profile is provisioned)
%  - Traffic


% vSIM, Device Profile Provisioning, and Run Time Operations.
In this Section, we detail the architecture of \PaperName{}, illustrated in Figure~\ref{fig:arch}.
At its core, \PaperName{} includes two key new innovations, 
First is the vSIM software and supporting capabilities that enable it to be trusted (Section~\ref{sec:arch:vsim}).
Second is the dynamic Device Profile Provisioning (Section~\ref{sec:arch:profile}), which is the unique capability we introduce that allows for a user to use different device profiles, which reduces an adversaries ability to track the users activity.
After detailing each of these, discuss the Run-Time operations (Section~\ref{sec:arch:runtime}), to illustrate how the 5G can work without modifications.  

\begin{figure} 
    \centering
    \includegraphics[width=\linewidth]{figures/arch.png}
    \caption{Architecture of \PaperName{} connected to 5G core network. }
    \label{fig:arch}
\end{figure}


\if{0}
At its core, \PaperName{} includes two key new innovations, 
First is the vSIM software and supporting capabilities that enable it to be trusted (Section~\ref{sec:arch:vsim}).  This is illustrated in Figure~\ref{fig:overview} as Components (1) and (2).  
Component (1) is the vSIM software, which executes on the device's main CPU within a TEE, providing hardware-enforced isolation between vSIM's secure execution and the operating system in the normal execution mode. vSIM implements standard SIM card functions for 5G authentication and adds secure provisioning capabilities. Component (2) is the trusted hardware, which includes keys which are used for authentication.
Second is the dynamic Device Profile Provisioning (Section~\ref{sec:arch:profile}), which is the unique capability we introduce that allows for a user to use different device profiles, which reduces an adversaries ability to track the users activity.
 This is illustrated in Figure~\ref{fig:overview} as Components (3), (4), and (5). 
Component (3) is the remote attestation, which measures the state of the hardware and signs it using platform private key to establish trust in the hardware.
Component (4) is the Profile Manager, residing on the provider's infrastructure. This component handles profile management and attestation verification for vSIM processes requesting new profiles.
Lastly, component (5) illustrates the successfully downloading of a profile, which vSIM stores permanently in secure storage.
We then discuss the Run-Time operations (Section~\ref{sec:arch:runtime}), to illustrate how the 5G can work without modifications.  
\fi



%In this section we describe \PaperName{} architecture in detail. \PaperName{} is composed of 5 key components (as illustrated in Figure~\ref{fig:overview}).
% illustrates the overview of \PaperName{} architecture. 
% In the figure, the blue arrow shows profile provisioning procedure and the red arrow shows authentication to network through subscriber profile credentials. 
%Component (1) in Figure~\ref{fig:overview}, is vSIM, which executes on the device's main CPU within a TEE, providing hardware-enforced isolation between vSIM's secure execution and the operating system in the normal execution mode. vSIM implements standard SIM card functions for 5G authentication and adds secure provisioning capabilities. Component (2) is the trusted hardware, which includes keys which are used for authentication. Component (3) is the remote attestation, which measures the state of the hardware and signs it using device private key to establish trust in the hardware.
%Component (4) is the Profile Manager, residing on the provider's infrastructure. This component handles profile management and attestation verification for vSIM processes requesting new profiles.
%Lastly, component (5) illustrates the successfully downloading of a profile, which vSIM stores permanently in secure storage.
 
% Diagram of arch.  

% Roles: HW Manufacturer (Intel/ARM/…) -- mention assumptions/requirements.  System Manufacture (Samsung, Apple, Google, Motorola)  -- mention assumptions/requirements (like put root certificate, which can validate the system manufacturer's public key).  Cellular Provider (AT&T, Verizon).  User (the consumer who owns the phone).

% Table with all of the keys (who created, where stored, and where used)?
\subsection{vSIM}
\label{sec:arch:vsim}

vSIM is a software-based implementation of SIM functionality.  
Like SIM and eSIM, it includes both a device and subscriber profile and  supports 5G authentication.  Where vSIM differs is in the addition of the ability to dynamically provision the device profile.   

As vSIM is executed in a secure enclave of a Trusted Execution Environment (TEE), the interface to the untrusted world is through ECALLs, which are used to call trusted functions from the untrusted application code, and OCALLs, which are used to call functions from the trusted code back into the untrusted application, with parameters passed as shared memory regions. The communication occurs through the Security Monitor (on the trusted world side) and the Security Monitor driver in the OS (on the untrusted world side). 
To illustrate, for authentication, vSIM supports the \emph{challenge()} call, which is called by the Authenticator module running in the non-secure world.  This function takes the \emph{RAND} and \emph{AUTN} parameters part of the 5G authentication process, as outlined in Section~\ref{sec:background}. 

Unlike the traditional SIM, vSIM includes the device profile provisioning capability.  This interface uses a proxy (Profile Manager Proxy) running in the non-secure world which interfaces with the Profile Manager in the Provider's infrastructure.  This proxy calls vSIM to first, establish a secure channel with \emph{establishSecureChannel()} and then \emph{addDeviceProfile()}. 



%vSIM is a software-based implementation that provides 5G functionalities equivalant to eSIM. It supports two primary capabilities: \textbf{(i)} Remote device and subscriber profile provisioning. \textbf{(ii)} Subscriber authentication to the network. Table~\ref{tab:vsim_interfaces} illustrates the interfaces vSIM is providing. For remote device and subscriber profile provisioning, there exists an entity on the untrusted world (e.g., in ME) that acts as a proxy between vSIM and the provider. vSIM opens an interface with this entity to exchange secure provisioning messages, and another interface exists between the proxy and the provider. These interfaces are used to establish a secure channel between vSIM and the provider and later for secure profile download and management. As we discuss later in~\ref{sec:arch:profile}, all sensitive cryptographic operations are done inside the vSIM and the proxy is not capable of eavesdroping or modifying the messages. Besides, vSIM opens a interface to ME for local profile management with the permissions specified in the GSMA standard~\cite{gsma}.
%The authentication mechanism maintains compatibility with existing eSIM procedures. vSIM opens a dedicated interface to the ME for authentication challenge-response exchanges. 

\if{0}
\begin{table}
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|c|c|p{2.4cm}|}
\hline
 & \multicolumn{2}{c|}{\textbf{Between}} & \textbf{Description} \\
\hline
\multirow{\parbox{2cm}{\textbf{Profile Management}}} & vSIM & Proxy Entity &  Provides a communication channel through which vSIM securely communicates with the provider. \\
\cline{2-4}
 & Proxy Entity & Provider & Forwards encrypted messages between vSIM and the provider. After etablishing secure channel, it handles secure profile download and management. \\
\cline{2-4}
 & vSIM & ME & To locally manage the subscriber profile with permissions specified in~\cite{gsma} \\
\hline
\textbf{Authentication} & vSIM & ME & To Exchange challenge-response messages to authenticate subscriber to the network. \\
\hline
\end{tabular}
\caption{Interfaces}
\label{tab:vsim_interfaces}
\end{table}
\fi


To ensure vSIM can be trusted, we rely on a secure boot process that establishes a chain of trust from hardware to application. The trust foundation begins with a firmware signing key pair, provisioned by the manufacturer: the firmware is signed using the firmware private key, and its authenticity is verified during boot using the corresponding firmware public key stored in hardware. In addition, a platform key pair (group keys as discussed in Section~\ref{sec:overview}) is provisioned offline by the manufacturer and securely embedded in hardware.

During boot, the zero-stage bootloader verifies the firmware’s integrity by checking its hash against the digital signature created with the firmware private key. Once validated, the security monitor, part of the trusted firmwarw is loaded as the only component with access to the platform private key. After vSIM is loaded, the security monitor records the state of the vSIM software and produces attestation evidence (signed measurements of the platform and vSIM) using the platform key pair. This attestation mechanism enables continuous trust verification of vSIM throughout its lifecycle, while enforcing strict access control. vSIM itself never has direct access to the platform private key.

% vSIM
%   - Runs in TEE
%   - Interfaces
%   - Just the application 
% Establishing Chain of Trust
%   - HW -> Boot Loader -> Security Monitor -> Driver (can take attestation measurement) -> Application (vSIM)
%   - Platform vSIM runs on (which is part of secure boot process)
%   - Secure Boot (to get to vSIM)
%       (Trust HW (group keys)
% Main subsection with details:

%     - vSIM SW (TEE stuff plus driver) -- multiple SIM
%     - Secure Boot
% 	- Provisioning a user profile (includes remote attestation)
% 	- 5G Authentication


\subsection{Device Profile Provisioning}
\label{sec:arch:profile}
% Device Profile Provisioning
%   - Provider SW component + UE Software component
%   - Remote Attestation
%   - Secure Channel Establishment
%   - Security Guarantees (inside threat model?)
%   - Device Profile Switching

Central to the privacy enhancements that \PaperName{} enables is the ability to dynamically provision a device profile.  Recall that a device profile consists of a device ID (EID) and a secret key (eSIM secret).  For an operator to provision this, the operator needs to attest that the software stack is as expected (and can be trusted), and then establish a secure channel to provision the profile.  We outline these here.

\subsubsection{Remote Attestation}
% Secure boot ensures that, at boot time, the intended software was loaded.  Remote attestation provides a means for a remote party to verify what is currently running on the valid and trusted platform -- so it can be sure only the intended software, and no additional applications have been added.  We do not consider the vSIM application to be part of the secure boot process, but something that may have different implementations that could be loaded. The vSIM remote attestation is a system level software that executes in the secure world and is part of the secure boot process. This process includes a procedure that can generate a cryptographically signed quote, asserting that vSIM is executing in a trustworthy manner. The quote is a hash of the vSIM state, i.e., its binary, signed by an attestation key that can be derived between the remote party communicating with the remote attestation service.

% Remote attestation provides the mechanism for the remote provider to verify the trustworthy of the previous components in the chain of trust through the target component's measurement~\cite{}.
% The verifier guarantees that the software can trust the current platform and that no malicious software has been loaded. 
% Remote attestation is the process of validation of a claim made by the target component's measurement[?].  
% vSim is an application that executes in a trusted enclave. We do not consider it as part of the secure boot; instead, it relies on the chain of trust built on top of the secure boot. The vSim needs to prove that the current hardware that it is running on, is a genuine vSim hardware. 
% In vSim, the following components can be remotely attested to: the physical hard device, Keystone secure monitor (SM), and vSim software. In a similar fashion, the Secure Monitor and vSim measurements(hash values) are attested to assert that vSim is executing in a trustworthy manner. 
To make sure that the provider is talking to an authenticated and verified piece of hardware and software, \PaperName{} also provides a way to attest its identity remotely. vSIM needs to prove that \textbf{(i)} It is currently running on a valid and trusted platform -- so the provider can be sure that the intended software is running. \textbf{(ii)} It is in a valid and unmodified state. To this end, vSIM responds to cryptographic challenges from the provider with the attestation quote. The quote includes the hardware state, which includes measurement of the Security Monitor (SM) and its signature, measurement of vSIM e.g., its binary and its signature. All this information is signed by the device's private key (which is part of a group signature key discussed in~\ref{sec:overview}) along with the challenge and sent to the remote verifier. The provider verifies the signature to confirm that the response originates from a genuine vSIM hardware and that vSIM is in a valid and trusted state. 


%Secure boot ensures that only authorized software is loaded and executed on the device during the boot time. We do not consider the vSIM application to be part of the secure boot process, but an application that runs inside the secure world and relies on the established chain of trust that secure boot creates. 

% In vSIM, multiple components can be remotely attested: \textbf{(i)} the physical hardware device, \textbf{(ii)} the TEE Secure Monitor, and \textbf{(iii)} the vSIM application itself. The attestation process verifies measurements of both the Secure Monitor and the vSIM application to ensure they have not been tampered with. This comprehensive verification ensures that the vSIM is executing in a trustworthy manner.

\subsubsection{Secure Channel Establishment}
\label{sec:arch:trust}


  \begin{table}
% \begin{figure*}
    \centering
 % \begin{minipage}[b]{0.5\textwidth }
 \begin{tabular}{ll}
        \hline
        \textbf{Notation} & \textbf{Description} \\
        \hline
         $n_X$ &  Nonce generated by party X \\
         $pk_P$ & Public key of the provider \\
         $sk_P$ & Private key of the provier\\
         $pk_D$ &\PaperName{} platform group public key\\
         $sk_D$ &\PaperName{} platform private key\\
         $d_X$ &  Ephemeral private key of party X \\
         $K_s$ & Ephemeral session key \\
         $ATTR$ & Attestation Request \\
         $Q_V$ & Attestation quote from vSIM \\
         \| & Concatenation \\
         $[D]_k$ & Encryption of message D using key k \\
         $\sigma(D)_k$ & Signature of D with key k \\
         
\hline
\end{tabular}
\caption{Protocol notation}
\label{tab:notation}
\end{table}
 % \end{subfigure}
 % \end{minipage}

 
 % \begin{subfigure}
% \begin{minipage}
     \begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figures/sec-channel.png}
    \caption{Secure Channel Establishment Protocol}
    \label{fig:sec-channel}
\end{figure}
 % \end{subfigure}
% \end{minipage}
% \end{figure*}


Before the provider is able to provision the device and subscriber profiles, it needs to ensure that it is talking to vSIM through a trusted channel. \PaperName{} assumes that the provider knows the valid state, i.e. the valid binary measurement of vSIM, and is able to verify its quote $Q_V$. Besides, the provider's private key, $sk_P$, and \PaperName{} platform private key $sk_D$ are securely provisioned into them and their public keys $pk_P$ and $pk_D$ (group public key as discussed in~\ref{sec:overview}) are available. \PaperName{} also assumes that it is able to securely generate random numbers, generate key pairs, and derive keys from the fused cryptographic keys. 

The process (shown in Figure~\ref{fig:sec-channel}) is initiated by the vSIM software. vSIM generates a random nonce $n_V$ as a challenge and a temporary Elliptic Curve (EC) private key $d_V$ and the corresponding public key $dG_V$ that are used to generate a session key. $d_V$ remains securely stored within vSIM's protected memory throughout the session. This information is inaccessible by any untrusted software to maintain session integrity. vSIM then encrypts $n_V$ and $dG_V$ using the provider's public key $pk_P$ and transmits it to the provider. In the next step, the provider receives and decrypts vSIM's request. The provider extracts $n_V$ and $dG_V$ using its own private key. The provider then generates its own random nonce, $n_P$, an ephemeral EC private key $d_P$, and its corresponding public key $dG_P$ and an attestation request vector $ATTR$. To authenticate itself to vSIM, the provider creates a signature of $n_V$, $dG_P$, $n_P$, $ATTR$, signed with $sk_P$ and sends it to the vSIM. It is worth noting that there is no need to protect these four, because without the knowledge of $d_V$ or $d_P$, an attacker can not proceed in the communication. In addition, the provider derives the shared session key $K_s$ through the Elliptic Curve Diffie Hellman (ECDH) process~\cite{haakegaard2015elliptic}. When the information is received on the vSIM side, it verifies the provider's identity by comparing the sent and received nonces $n_V$. vSIM then derives the shared session key $K_s$, through ECDH using its private key $d_V$ and the provider's public key $dG_P$.
 vSIM then invokes the attestor component (in Security Monitor) with the challenge in the attestation request vector (to include it in the attestation response and to ensure its freshness) to generate the quote $Q_v$ signed by the \PaperName{} platform secret key $sk_D$, and then concatenates the quote with the nonces $Q_V || n_V || n_P$. vSIM then encrypts this concatenated value using the derived session key $K_s$ and transmits it back to the provider. Finally, the provider decrypts the response using $K_s$ and extracts the vSIM quote $Q_v$ along with the nonces. It then validates the attestation by recomputing the expected quote based on the challenge parameters it originally sent and \PaperName{} group public key $pk_D$ and comparing the result against the received quote. If the quotes match, the provider verifies the freshness of the message by checking the included nonce values. Upon successful verification of both the attestation and freshness guarantees, the provider sends an acknowledgment to vSIM, announcing that the secure channel is established.

After establishing a secure channel, the provider sends a genuine device profile 
%along with the long-term secret key 
to the ME, which is handled by vSIM decrypting and securely storing it. To ensure the confidentiality and integrity of sensitive information such as authentication keys, attestation keys, subscriber identification, and other 5G security parameters, they are all stored using a secure storage device. The \textbf{secure storage} guarantees exclusive access for each trusted application to its own secure objects. This form of storage provides a private location for trusted applications, such as vSIM, to place their critical information. 
% that is inaccessible to other trusted applications and system software running in the normal world.




% \subsubsection{Security Guarantees}
% The proposed \PaperName{} architecture is designed around the following security guarantees:

% \textbf{Mutual Authentication.} Both entities are authenticated through challenges to defend against impersonation attacks.

% \textbf{Mutual Non-Repudiation.} By providing signatures, none of the entities can later deny participation in the protocol.  

% \textbf{Forward Secrecy.} In the beginning of each session, a new session key is derived (using ephemeral EC keys of the entities) to defend against previous session key compromise.

% \textbf{Freshness.} New attestation challenges and nonces are generated in each session to defend against replay attacks.

% \textbf{Confidentiality and Integrity.} Session key establishment defends against eavesdropping or tampering of messages.

% \textbf{Trust Assurance.} Finally, the provider can trust vSIM by verifying its state through a valid attestation quote, defending against the possibility of a compromised vSIM environment.


\subsubsection{Switching Between Profiles}
Finally, \PaperName{} can switch between profiles without exposing an identity linkage. As a simple proof-of-concept, we implement vSIM with the capability to store multiple profiles simultaneously and seamlessly switch between them. As specified by the GSMA standard~\cite{gsma}, different profiles on the same device are isolated from each other. To this end, nested enclave are the ideal architecture to isolate each profile in a child enclave of vSIM. This approach depends on the architecture of the TEE and whether it supports nested enclaves. Park \emph{et.al.} proposes a nested-enclave solution for Intel SGX to achieve similar isolation guarantees~\cite{9138984}, which we will explore as future work.


\subsection{Run-time Operation}
\label{sec:arch:runtime}

% Run-time Operation
%  - 5G Authentication (assume device profile is provisioned)
%  - Traffic 

vSIM aims to have the same security guarantees and operation as a physical SIM card once provisioned---since, at that point, the security model remains the same. The SIM functions as a root-of-trust for mobile communications needed for authentication by securely storing both the device profile and the subscriber profile information, such as the long-term secret key \textit{(k)} and the IMSI. This security property extends to the vSIM implementation, and here we overview vSIM in operation after the device profiling stage. 

\textbf{Subscriber Profile Provisioning:} 
The SIM functions as a root-of-trust for mobile communications needed for authentication by securely storing the device profile.  This is central to then including being able to provision a subscriber profile, 
information, such as the long-term secret key \textit{(k)} and the IMSI.
We note that, the long-term secret key is only provisioned after establishing trust of the device and its software  (discussed in Section~\ref{sec:arch:trust}), at which point vSIM is equivalent to having a physical eSIM card.  
 
\textbf{5G Authentication:}
With a subscriber profile provisioned, the user can then connect to the network.  
When they do so, the 5G authentication process begins as specified in the 3GPP Specification~\cite{3gpp_ts_33_501}. Similar to the traditional process, the Mobile Equipment (ME) forwards the challenge to vSIM. Upon reception of the challenge, vSIM retrieves the long-term secret key (previously received from the provider) from its secure storage using the corresponding ID. Then vSIM generates the necessary cryptographic keys and a response. Once the keys and response are generated, vSIM securely transmits them back to the ME, which in turn sends them to the network provider for verification. 

\textbf{Traffic: } 
After the authentication process, the phone is connected to the network and a vSIM (or any SIM) is no longer needed.  At this point the operator will have stored information about the state of that subscriber, indicating that it is now authenticated, and information about it that will allow it to identify traffic from that subscriber.  The software on the user equipment (phone) will store this in non-secure world, and include in data traffic headers.  

   








==> sec/eval.tex <==
\section{Evaluation}
\label{sec:eval}

With \PaperName{}, there are three key questions.  (i) does it provide suitable privacy enhancements, (ii) is it compatible with 5G software and protocols, and (iii) what, if any, overhead does this extra capability encur.  After describing our experimental setup, we answer each of these questions.


\subsection{Experimental Setup} 
We use Xilinx Genesys2 FPGA board with 1GB 1800Mbps DDR3, programmed as discussed in Section~\ref{sec:prototype}. We ran srsUE in an untrusted Linux environment alongside the vSIM, which is secured within the Keystone trusted execution environment. The board connections are established through a dedicated Ethernet hub with no additional devices attached to minimize network overhead and ensure consistent performance measurements. The srsRAN software, profile provisioning operations, and containerized 5G core network components are hosted on a personal laptop. All system components are connected to the same network switch and communicated within a local network environment. For , we run the server program in a C6220 Cloudlab~\cite{cloudlab} Node with an x86-64 architecture, 8 Intel E5-2650 CPU cores, and 65GB of RAM. 

\subsection{Privacy}

%\textbf{Correlation Attack.} 

A core principle in \PaperName{} is the by decoupling the device profile (which includes the EID) from the user identity, we enhance privacy such that an operator cannot correlate online clients, and by extension, track a user's online and physical activity.  
Different techniques have been used to correlate online clients. 
% These include traffic/website fingerprinting~\cite{}, flow correlation~\cite{}, and graph-based analysis~\cite{}. 
Although obfuscation can help mitigate these attacks, most of them still work well against many obfuscation techniques (as discussed in ~\ref{sec:background}). Here, we demonstrate through evaluation the privacy benefits that vSIM provides by significantly reducing the effectiveness of these attacks compared to systems without vSIM.


SiamHAN~\cite{cui2021siamhan} is a sophisticated graph-based model that performs accurate user flow correlation. In SiamHAN, the attacker first builds a knowledge graph and then using the SiamHAN model, it can determine if an IP belongs to a specific user. SiamHAN processes knowledge graphs and generates comparable embeddings. The system then calculates a Euclidean distance between these embeddings to determine whether two addresses belong to the same user. What we are trying to show is that in such correlation systems, a hardware-based feature like EID can easily make different flows distinguishable, by reducing the distance of flows that are generated from the same hardware.

We simulate SiamHAN on a network with vSIM-enabled devices and compare it against a version without vSIM. We modify the test dataset to include the EID feature across both scenarios. In the vSIM-protected implementation, different EIDs are assigned to each IP address in the network, regardless of whether multiple IPs belong to the same user device. In contrast, the unprotected implementation maintains shared EIDs for IPs originating from the same device, mirroring current SIM design. To measure the effectiveness of vSIM, we focus our analysis specifically on scenarios where a single user/device uses multiple IP addresses. We exclude users with only one IP address from our evaluation, as these cases would not demonstrate the correlation protection capabilities we aim to assess. Our experimental results reveal a significant privacy improvement: the accuracy of correlating IPs in a network with \PaperName{} protected devices drops to 75\%, while the network without \PaperName{} achieves a much higher correlation accuracy of approximately 94\%. 

To further investigate vSIM's effect on such models, we integrate our system with network obfuscation techniques. 
Network obfuscation can be implemented in various ways, 
% ranging from generating fake traffic data~\cite{} to employing traffic mimicry techniques~\cite{}. 
For our experiment, we specifically modify the TLS-related fields. The results (Table~\ref{tab:acc}) show that when vSIM is combined with obfuscation techniques, correlation accuracy drops dramatically to 49\%. However, without vSIM, the SiamHAN model remains highly resistant to the same obfuscation techniques, maintaining accuracy of 91\%. This difference demonstrates that vSIM creates a powerful synergy with obfuscation methods and significantly amplifies their effectiveness against sophisticated correlation attacks. This combined approach represents a much more robust privacy protection strategy than applying either technique in isolation. 
%The accuracy comparison is illustrated in Table~\ref{tab:acc}.
\textbf{\begin{table} [h]
    \centering
    \caption{Accuracy comparison of running SiamHAN model on a network with and without vSIM}
    \begin{tabular}{|c|c|}
    \hline
         &  \textbf{Accuracy} \\
    \hline
         \textbf{vSIM} & 75.0\%   \\
         \textbf{Without vSIM}  & 94.3\%  \\
         \textbf{vSIM + obfuscation}  & 49.3\% \\
         \textbf{Without vSIM + obfuscation}  & 91.4\% \\
    \hline
    \end{tabular}
    \label{tab:acc}
\end{table}}


\begin{figure} 
    \centering
    \includegraphics[width=\linewidth]{figures/accuracycomparison.png}
    \caption{Comparison of SiamHAN model accuracy across different privacy configurations and client group sizes. The graph illustrates performance under four distinct scenarios: implementation without vSIM, with vSIM, combined approach with TLS parameter obfuscation and vSIM, and without vSIM.}
    \label{fig:model}
\end{figure}

Figure~\ref{fig:model} illustrates the accuracy of the SiamHAN model with and without vSIM, as well as when integrated with obfuscation techniques, across different numbers of clients. The results show a substantial performance gap between vSIM-protected and unprotected systems, even when analyzing small client groups. This consistent effectiveness across varying client population sizes demonstrates that vSIM provides robust privacy protection regardless of network scale which makes it a reliable defense mechanism against sophisticated correlation attacks in both small network environments and larger ones.



\subsection{Compatibility}


With the implementation discussed in~\ref{sec:prototype}, we successfully validate that the UE can authenticate with the network and transmit data seamlessly. When the UE initiates a connection to the network, it receives an authentication challenge from the 5G core to verify its identity. The UE then forwards this challenge to the \PaperName{}, which performs the necessary cryptographic calculations to generate the appropriate challenge response. This response is then returned to the UE, which forwards it to the network to complete the authentication process. After successful authentication, all subsequent connection and communication procedures continue according to standard protocols. This experiment shows that, the proposed architecture maintains compatibility with existing network infrastructure.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/nas-crop.png}
    \caption{Packets exchanged between vSIM and 5G core during UE successful authentication to the network. The red box in the lower left indicates the authentication response parameters calculated by the vSIM.  }
    \label{fig:nas}
\end{figure}

Figure \ref{fig:nas} illustrates the packet exchange between vSIM and the 5G core network during UE authentication. The bottom highlighted red box indicates the authentication response parameters calculated by vSIM and transmitted to the 5G core. Upon successful verification of these authentication parameters, the 5G core completes the registration process by sending registration accept and registration complete messages to the UE.


\begin{figure}[ht]
    \centering
    % \begin{subfigure}{0.45\textwidth}
    \subfloat[]{%
        \includegraphics[width=\columnwidth]{figures/n1.png}%

        }%
        % \end{subfigure}
        \\
    \subfloat[]{%
       % \hfill
    % \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\columnwidth]{figures/n2.png}%
        }%
        % \end{subfigure}
  
    \caption{Network usage of UE. (a) With vSIM, (b) Without vSIM}
            \label{fig:net}
\end{figure}

 The 5G authentication process is done only once when the UE wants to attach to the network, and therefore communication can occur without vSIM's involvement afterwards. To demonstrate, we setup an iperf3 server on the 5GC machine and a client on the \PaperName{} prototype that runs UE. UE sends TCP traffic to the network both with using vSIM and without vSIM. Figure \ref{fig:net} (a) illustrates the network usage rates using vSIM, and Figure~\ref{fig:net} (b) shows it with USIM.  Apart from some noise, they are roughly identical, illustrating the fact that there is no overhead.

\subsection{Performance}

To ensure reliable measurements, we repeat each experiment 10 times and report the average values. First, we measure the complete end-to-end device profile provisioning process time. This measurement includes the processing time required by both \PaperName{} and the provider to generate and verify each message in the protocol sequence, plus the round-trip network transmission time that accounts for all communication latency. 


\textbf{Secure Channel Establishment.}
The \PaperName{} secure channel establishment protocol for device profile provisioning executes in approximately 805 milliseconds for the complete round-trip operation. This total time includes TCP/IP socket establishment and termination, message reception and parsing from the provider, message encryption and decryption operations, context switches between secure and normal worlds, and digital signature generation and verification including quote processing. 

For the remote attestation process, we measure the time required to prepare the quote (excluding verification), which takes approximately 19 milliseconds. This operation includes generating the hash of the security monitor and enclave binary, creating the attestation structure, and producing the signature using the private key. On the provider side, the verification process consists of a direct comparison between the received attestation quote and the expected signature value based on the known-good enclave measurement. 

\textbf{UE attachment to network.}
Since vSIM runs inside an enclave, starting the enclave for each authentication adds significant latency. To address this, we initialize the enclave when the UE starts. Our measurements show that computing the challenge response inside the enclave takes only 5 milliseconds. However, when integrated with the UE, the total time to transmit the challenge vector to vSIM and receive results through the shared memory channel increases to approximately 658 milliseconds. For comparison, authentication without vSIM takes about 7 milliseconds. This increase in authentication time with vSIM can be attributed to the overhead of preparing data for secure communication and formatting the response vector between components, secure world context switches between normal and trusted environments, and the execution of multiple communication and computation functions to process the authentication vector. This time only corresponds to the period required to generate the authentication response vector, since the remaining processes—such as transmitting the response to the core network and deriving the 5G keys in the ME—remain identical between vSIM and standard implementations (see results on Table ~\ref{tab:auth}).

\begin{table}
    \centering
    \caption{Latency comparison of authentication with and without vSIM in milliseconds}
    \begin{tabular}{|c|c|}
    \hline
         &  \textbf{Time (ms)} \\
    \hline
         \textbf{UE + vSIM} & 658.9   \\
         \textbf{UE + without vSIM}  & 7.6  \\
         \textbf{vSIM only}  & 5.2 \\
    \hline
    \end{tabular}
    \label{tab:auth}
    
\end{table}
\vspace{0.2in}
\begin{figure}
    \centering
    % % \begin{subfigure}{0.45\textwidth}
    % \subfloat[]{%
    %     \includegraphics[width=.51\columnwidth]{figures/vue_cpu_cdf.png}%

    %     }%
    %     % \end{subfigure}
    % \subfloat[]{%
    %    % \hfill
    % % \begin{subfigure}{0.45\textwidth}
        
    %     }%
    %     % \end{subfigure}
    \includegraphics[width=1\columnwidth]{figures/vue_cpu_cdf_comparison.png}%
  
    \caption{CPU usage CDF of UE. (a) With vSIM, (b) Without vSIM}
            \label{fig:cpu}
                
\end{figure}

\vspace{0.1in}

As part of the resource analysis, we measure the CPU and memory usage for UE implementations with and without vSIM. We collect these performance metrics by 
leveraging the hardware counters on the board for both memory and cpu. 
% directly reading system data from the \textit{/proc/} directory. 
Figures \ref{fig:cpu} (a) and (b) present the CPU usage cumulative distribution function (CDF) for UE with and without vSIM, respectively.There is no significant difference in CPU utilization between the two implementations.

\begin{figure}[ht]
    \centering
    % \begin{subfigure}{0.45\textwidth}
    % \subfloat[]{%
    %     \includegraphics[width=.51\columnwidth]{figures/vsim_memory.png}%

    %     }%
    %     % \end{subfigure}
    % \subfloat[]{%
    %    % \hfill
    % % \begin{subfigure}{0.45\textwidth}
    %     \includegraphics[width=0.51\columnwidth]{figures/esim_memory.png}%
    %     }%
    %     % \end{subfigure}
     \includegraphics[width=1\columnwidth]{figures/u_memory_comparison.png}%
  
    \caption{Memory usage of UE over time. The green line is with vSIM and the purple line is without vSIM.}
            \label{fig:mem}
                   
\end{figure}





Figures~\ref{fig:mem} a and b show the memory usage patterns of UE with and without vSIM throughout the execution period. The measurements reveal less than 1\% memory overhead when using vSIM compared to the baseline implementation, which is attributed to the additional memory requirements of vSIM and the shared memory channels established for secure communication.

\textbf{Profile Switching.} Switching between different device profiles requires re-authentication of the profile to the network. From the vSIM perspective, there is no additional latency when switching between profiles. Unlike eSIM, which typically allows only one (or in more recent designs, two) subscriber profiles to be enabled simultaneously (with a fixed device profile), vSIM can have multiple device and subscriber profiles enabled concurrently. Consequently, the latency of profile switching corresponds solely to the time required for the UE to deregister from the network, reinitialize the Non-Access Stratum (NAS) stack, and re-authenticate to the network. We measured this total profile switching time to be 1681.8 milliseconds.  We see this as a opportunity for optimization as future work.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{ltest.png}
    \caption{Latency of authenticating a UE by 5G Core with different number of concurrent requests. The orange line is using 1 gNodeB and the green line is using 2 gNodeBs with even loads.}
    \label{fig:placeholder}
\end{figure}



==> sec/overview.tex <==
%   Diagram: EID_OBFS (a) nodes with shared identifier EID and then obfuscation, (b) vsim with multiple idetifiers, each with obfuscation.


\section{\PaperName{} Overview}
\label{sec:overview}


%IMSI tied to subscriber, and uniquely identifies subscriber, but there is no tie between IMSIs.

%Note: we assume the IMEI can change.

% 	- Given that the fixed key is the problem, we look to break that -- reference Diagram EID_OBFS (b).  Emphasizing how this provides privacy
% 	- We introduce vSIM -- sw that provides similar functionality as SIM, but without the reliance on a pre-shared key (at manufacturing time).
% 	- Overview: Run vSIM in a trusted enclave.  Extend definition of user profile to include the long-term private shared key (in addition to IMSI, and subscriber info). 
    
%     To do this, we need to establish trust:

% 	- Trust the Hardware
% 		○ Group keys
% 	- Trust the software
% 		○ TEE
% 		○ Remote Attestation
%             oen - two overview talkig about what it is.


% (Somewhere mention we assume you can change the IMEI, which I think is like a MAC address, that is tied to the modem, but there are models which it can be changed)

To address the lack of privacy in 5G communications, we introduce \PaperName{} and vSIM.  
vSIM is a software-based SIM implementation that enables secure device profile provisioning (in addition to remote subscriber profile provisioning, which carries over from eSIM capabilities).  
\PaperName{} is the overall architecture, which includes vSIM and associated infrastructure to support trusted dynamic provisioning of device profiles.

%To address the lack of privacy in 5G communications, we introduce vSIM, a software-based SIM implementation that enables secure device profile provisioning (in addition to remote subscriber profile provisioning, which carries over from eSIM capabilities).  
%The EID device identifier (and tightly coupled eSIM secret key provisioned at manufacturing time) is integral to the 5G authentication process.
%However, having this fixed identifier enables all traffic to be associated with a specific node regardless of any obfuscation used.  
%But, binding a fixed secret key and device identifier along with a subscriber identifier to a SIM Card is a source of privacy concerns. These credentials, used to establish secure channels with profile management servers, create a permanent binding between the subscriber profile and the hardware identity and make them easily correlatable. 

vSIM decouples the subscriber identity from the device, allowing a node to have multiple device profiles, and therefore multiple EIDs (the device identifier currently hard coded in eSIMs), as shown Figure~\ref{fig:nodes}(b). This separation allows the system to have traffic flows that cannot be easily correlated (e.g., an attacker sees flows f1 and f4 coming from different devices, not just different subscriptions from the same device).
Note, the International Mobile Equipment Identity (IMEI), is another identifier that can compromise privacy.  We leverage the fact that this identifier is programmable in many modems, so it can be changed at runtime~\cite{imei}.


% \textcolor{red}{The proposed mechanism defends against an attacker that can: (1) eavesdrop on the messages exchanged between vSIM and the provider, (2) impersonates as an endpoint by replaying legitimate messages, (3) replays a previously stolen session key for future communications.}


%\subsection{Building Trust}

The ability to provision device profiles at runtime, addresses the privacy concern, but opens a new key challenge: trust establishment.  In eSIM, a pre-shared key and device identifier (established during manufacturing) is the means by which trust is established between the operator and device.  In vSIM, trust is established through four existing mechanisms, described below.  

%attestation that proves the execution of specific trusted software. This trust establishment follows a chain of trust that originates from a hardware root-of-trust.







\textbf{Trusted Execution Environment (TEE)}: In order to isolate the execution of the vSIM from other system software,
vSIM is intended to run in a trusted execution environment
(TEE). In traditional processors, an Operating System has
complete control over the system. It can, for example, inspect and modify any memory, including memory used by applications. This ability poses a threat as the information used in a
SIM card is intended to not be readable by the system. A TEE
is a hardware construct that is supported by modern processors (RISC-V Keystone~\cite{lee2019keystone}, ARM TrustZone~\cite{alves2004trustzone}, Intel SGX~\cite{intelsgx}, Intel TDX~\cite{inteltdx}, etc.)
and provides the ability to execute software in an isolated
manner, enforced by hardware. With this isolation, there are two execution modes: ``secure world'' and ``normal world''. vSIM executes in the secure world, and the operating system
(and other software) executes in the normal world. The normal world cannot access the secure world memory, and as a result vSIM's data in memory is isolated. 

\textbf{Remote Attestation:} 
 Physical SIM/eSIM cards establish trust by way of the manufacturing process and business relationships. As vSIM is software, we need a way for the mobile operator, or any entity provisioning data to the vSIM, to be able to trust that it is
interacting with vSIM software that is operating in a secure,
isolated manner (inside TEE), and that has not been modified. The vSIM builds
trust through secure boot and remote attestation. Secure boot
provides the foundation by creating a chain of trust where
each boot layer verifies the next layer’s signature, ultimately
ensuring the TEE and attestation system boot securely. The
attestation system, running within this verified TEE environment, then generates cryptographically signed quotes that
prove the integrity and authenticity of vSIM to remote parties.


\textbf{Group Key Scheme}: 
It is crucial in the design of vSim that no hardware information (e.g., cryptographic keys) is shared with any third party(including the remote authority) to preserve the user's privacy.  During remote attestation, one of the verifier's tasks is to authorize the hardware device to ensure that the software runs on ``genuine vSIM'' hardware and can, therefore, be trusted.  However, the remote authentication should occur in such a way that the verifier cannot identify the user's device.  

To achieve this goal, we design vSIM to use a group key scheme based on the direct anonymous attestation scheme (DAA)~\cite{10.1145/1030083.1030103}. DAA is based on the idea that a set of devices can be part of a group which can create the same signature without revealing which device in the group created~\cite{10.5555/1754868.1754897}. Each device has a unique cryptographic public-private key in a traditional digital signature scheme.  
However, in DAA, each device holds a unique private key (the platform private key) that is cryptographically associated with a common group public key (the platform public key) used for verification~\cite{alsouri2010group,chen2022mage,scarlata2018supporting}. DAA has been widely applied in scenarios similar to vSIM, where a device has to prove it is part of the group while preserving its anonymity—for example, Intel’s Enhanced Privacy ID (EPID) scheme~\cite{johnson2016intel}.
% It is important to note that anonymity is not revocable, but it allows for the detection of ``known'' keys, but it is outside the scope of this paper.




\textbf{Secure Boot}: All modern cell phones have a boot sequence that is layered into a small building step that brings up the system.  Each layer, regardless of the hardware manufacturer or the software running on the hardware, is subject to compromise if preventive measures are not taken.   The boot sequence includes a boot vector that is the starting point for each core. The program located at the boot vector is a very small program called the Zero-Stage-Boot-Loader (ZSBL) that is fused into the silicon (BootROM) to start the boot process.  On a hard reset, each core begins executing the instructions from the boot vector.  The main objective of the ZSBL is to load the firmware, which contains the First-Stage Bootloader (FSBL) and some optional data that might be required to complete the boot process.  To make progress, the  ZSBL has to manage all the available cores (each core comes online independently) and initialize the minimum I/O needed to load the firmware stored on an external device (e.g.  SDCard or BIOS) into main memory.  The control is then passed to the First-Stage-Bootloader, which loads the Secondary-Stage-Bootloader or the Operating System.

If an adversary has access to the external device where the firmware is stored and can change the firmware, it can compromise the system even before the operating system is loaded.  The adversary's objective is to blend the malicious firmware so that the operating system is opaque to its existence and is, therefore, very hard to detect. To prevent this type of compromise, a secure boot process can be used. 
% This type of attack has increased dramatically as more devices are connected to the internet.  Adversaries have focused on this type of attack because it gives them full control of millions of devices on the internet.
 
Secure boot is the process of bringing up a system in such a way that it guarantees that once the boot process has been completed, the system has not been compromised in any way and that only authenticated software has been used during the boot process. The secure boot process fuses the Zero-Stage-Bootloader(ZSBL) into the silicon to establish the root of trust. To ensure the fused in code is the correct code, the device includes a cryptographic key fused into the silicon with which it signs the ZSBL~\cite{maes2012pufky,bhargava2014efficient}. Starting at the ZSBL, each layer measures and endorses the next layer until control is handed over to the operating system.  To measure the next layer, the current trusted layer verifies the next layer with the next layer’s digital signature and public key to ensure that the image has not been modified.  If the measurement fails (the stored signature differs from the computed signature), the boot process halts, preventing the loading and execution of malicious software.  Otherwise, the current layer will endorse the next layer by signing the next layer with its private key before transferring control to the next layer, see Figure~\ref{fig:bootsequencecot}.  
    

\begin{figure} [t]
    \centering
    \includegraphics[width=\linewidth]{figures/secureboot_cotv3.pdf}
    \caption{Secure Boot and Chain of Trust.}
    \label{fig:bootsequencecot}
\end{figure}


==> sec/prototype.tex <==
\section{Prototype}
\label{sec:prototype}



We leverage Keystone~\cite{lee2019keystone}, an open-source TEE based on the Rocketchip RISC-V architecture~\cite{Asanović:EECS-2016-17}, which serves as our chosen TEE foundation. The prototype is a co-design of hardware and software. We implement vSIM to be run as an application inside the secure world. In the rest of this section we dive deeper into details of the prototype implementation. 


\subsection{Hardware}

We extend the Rocketship, an open-source System-on-Chip generator, along with the Berkeley Rocket Core, a synthesizable and parameterizable open-source RV64GC RISC-V core~\cite{Asanović:EECS-2016-17}.  The chip generator is built using Chisel, a high-level hardware construction language derived from the Scala language that emits synthesizable RTL.  We leverage the RocketChip generator to generate the modified cores, caches, memory controller and interconnects to design an integrated SoC.  Figure~\ref{fig:vsim_hardware} shows the changes we made to the generic Rocketchip SOC.  In addition to the changes, we add a cryptographic engine responsible for all encryption and hashing functions. We  also include the secure storage device to store the long-term keys (keystore 2).  We choose to store the cryptographic key (keystore 1) into the bootRAM logic.  In a commercial environment, this component would be replaced by a keystore such as an eFuse memory region for storing cryptographic keys.  The prototype also relies on the RISC-V physical memory protection standard (PMP)~\cite{riscv_ismii}, which enables the isolation of memory-mapped regions at runtime.  The memory map is shown on the right side of Figure~\ref{fig:vsim_hardware}. The PMP allows for specific memory regions to have their own permissions, such as the BootROM memory region being isolated by PMP entry 1, and therefore, only cores in machine mode can read from that memory address.


\subsection{Secure Boot Sequence}
In this section we describe how the secure boot mechanism works in the \PaperName{} prototype to establish the trust chain.  On a hard reset, all the cores in the system on chip (SoC) start reading and executing from the boot vector in the BootROM.  The program located at the boot vector is the Zero-Stage Bootload (ZSBL).  This first stage forms part of the Root of Trust as we trust the hardware and the ZSBL as it is part of the trusted boundary.  One of the cores (normally core1) is designated to load firmware from the storage device (SDCard) into the main memory (DRAM) and prepare the system for the next boot stage.  The firmware in \PaperName{} includes the First-Stage-Bootloader (FSBL), a signature of the firmware, and an operating system (Linux) with a root filesystem.  The firmware developer's private key signs the FSBL.
% ; in this case, it is also the device manufacturer. 
The firmware public key is shared with the device manufacturer and fused into the SoC.   
The ZSBL reads the firmware measurement by computing the 
FSBL hash and comparing the hash by decrypting the signature of FSBL with the firmware public key.  If the hash values do not match, the system jumps to the boot vector, effectively resetting the device. However, if the measurement is successful, and the boot process continues by endorsing (signing with device private key) the FSBL (see \ref{fig:secureboot_sequence}).  The FSBL used in vSIM is a modified version of OpenSBI that includes the Keystone Security Monitor~\cite{lee2019keystone}, forming the basis of \PaperName{} Trusted Execution Environment (TEE).  Control is transferred to OpenSBI, which executes the Security Monitor (SM).  The SM is responsible for initiating the physical memory protection (PMP) primitive of RISC-V for each core.  It includes a PMP entry that will protect itself even from the operating system.
% (see figure riscv yellow region).  
OpenSBI handles the rest of the boot process by handing it over to the operating system.  It is important to note that up to this point, all the cores run in machine mode (m-mode), the highest privilege level in the RISC-V architecture and part of what is considered to be the secure world.  As part of the handing over,  the privilege level of the cores is changed from machine mode to supervisory mode.  Therefore, when the operating system starts executing, it will run in supervisory mode and only have memory access to the memory region assigned to it by the security monitor.

\begin{figure} [ht]
    \centering
    \includegraphics[width=\linewidth]{figures/secureboot_sequencev3.pdf}
    \caption{Secure Boot sequence}
    \label{fig:secureboot_sequence}  
\end{figure}

\subsection{Security Monitor} 

The security monitor leverages the PUF and TRNG to derive an ephemeral key that is used by the chain of trust when performing local attestation. This allows vSim to be unlinkable and unclonable.

Furthermore, we leverage Keystone as a TEE.  Keystone’s security monitor enforces TEE guarantees and is the only process that runs in machine mode.  It is responsible for managing the PMP's configuration and address ranges, controlling the hardware delegation of the interrupts and exceptions in the system and providing a programmable interface\cite{lee2019keystone}.


During the remote attestation, the security monitor measures the security monitor and the vSIM enclave and signs the measurements(quote) with the platform's private key.  Only the security monitor can access the private key, and the remote verifier can only attest to the quote's validity if a valid platform private key signed the quote.

    
\begin{figure} [ht]
    \centering
    \includegraphics[width=\linewidth]{figures/Prototype_.pdf}
    \caption{Hardware prototype and Memory-Map}
    \label{fig:vsim_hardware}  
\end{figure}

\subsection{vSIM}
vSIM in implemented using the C language to run inside a Keystone enclave. At runtime, Keystone relies on Eyrie~\cite{lee2019keystone} runtime to execute enclave applications. We port the Libsodium~\cite{libsodium} library into the enclave for cryptographic operations. The prototype system uses \textit{X25519} elliptic curve cryptography, which is based on \textit{Curve25519} in Montgomery form, for key exchange~\cite{turan2019compact}. For digital signatures and quote signing, we implement Ed25519, which generates 64-byte signatures~\cite{bisheh2021cryptographic}. 
The implementation uses the \textit{XChaCha20-Poly1305} IETF authenticated encryption algorithm, which combines the \textit{XChaCha20} stream cipher with the \textit{Poly1305} message authentication code~\cite{thara2020survey}. We use standard 24-byte nonces for each encryption operation. Each encrypted message includes a 16-byte authentication tag for integrity verification, with messages padded to fixed 32-byte boundaries to prevent length-based information leakage. All hash operations use SHA-256. 

For authentication, we implement the standard XOR operations as specified in 3GPP-TS 33.501 standard ~\cite{3gpp_ts_33_501}, MAC verification, and SQN comparison using Tiny-AES~\cite{tiny-aes} library in the enclave. In accordance with the standard \cite{3gpp_ts_33_501}, we implement 5G authentication using Milenage algorithm suite with a 256-bit long-term secret key~\cite{yoo2019design}. 

Since it is not feasible to modify a commercial SM-DP+ server for profile provisioning, we emulate the server to implement the secure channel establishment. We implement it as a C++ based web server that contains a Remote Attestation Authority, which is responsible for verifying the attestation quote of vSIM. This Authority generates attestation challenges and keeps the valid state of vSIM to verify received quotes. For validation, it performs a comparison between the expected measurement hash and the received one. The server leverages the Libsodium~\cite{libsodium} library for cryptographic operations, which utilize the best available cryptographically secure random source provided by the underlying platform. 

To verify that vSIM seamlessly integrates with 5G infrastructure, we leveraged srsRAN \cite{srsran_docs} along with srsUE as our prototype UE and extend its source code with a new interface to communicate with the vSIM instead of the USIM. In the absence of radio hardware support, srsUE can establish a connection with srsRAN using ZeroMQ \cite{zeromq}, a high-performance asynchronous messaging library.

For the 5G Core Network (5GC), we employ Open5GS \cite{open5gs}, an open-source implementation of the 5G Core and Evolved Packet Core (EPC). srsRAN establishes a connection with the Access and Mobility Management Function (AMF) in the 5G Core network. The AMF is responsible for subscriber authentication, authorization, and mobility management.


